SCALE-VLP: Soft-Weighted Contrastive Volumetric Vision-Language Pre-training with Spatial-Knowledge Semantics

Vision-language models (VLMs) have demonstrated strong cross-modal capabilities, yet most work remains limited to 2D data and assumes binary supervision (i.e., positive vs. negative pairs), overlooking the continuous and structured dependencies present in volumetric data such as CT. Existing approaches often treat volumetric scans as independent 2D slices, compromising spatial coherence and underutilizing rich clinical semantics. We propose SCALE-VLP, a soft-weighted contrastive vision-language pre-training framework that integrates (i) volumetric spatial semantics to preserve anatomical structure and (ii) domain-aware, knowledge-infused semantics (e.g., radiological ontologies) to guide alignment. This yields structurally consistent and semantically grounded representations under limited supervision, demonstrating strong cross-task transferability (retrieval, report generation, and classification), and cross-domain generalizability with consistent gains without further fine-tuning. In particular, compared to the previous state of the art, SCALE-VLP achieves up to 4.3x higher top-1 CT-report retrieval, improves abnormality classification by 10 points, and reaches ROUGE-L 0.44 and BERT-F1 0.89 for report generation. Further, in zero-shot evaluation on an out-of-domain external dataset, we observe consistent gains, indicating the cross-task and cross-domain generalization ability of SCALE-VLP.

==> iclr2026/LaTeX/Figures/interpretation.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{iclr2026/LaTeX/Figures/similarity.pdf}
  \caption{Similarity Matrices by Model and Cluster. Panels (b–c) share axes: x = report embeddings; y = CT scan embeddings. }
  \label{fig:experiment-int}
\end{figure}


==> iclr2026/LaTeX/Figures/similarity.tex <==
% \begin{figure*}[htbp]
%     \centering
%     \begin{minipage}[t]{0.30\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{AuthorKit26/AnonymousSubmission/LaTeX/Figures/3D.png}
%         \caption*{(a) Kaleido-Med}
%     \end{minipage}%
%     \hspace{+0.1mm}%
%     \begin{minipage}[t]{0.3025\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{AuthorKit26/AnonymousSubmission/LaTeX/Figures/Clip.png}
%         \caption*{(b) CT-CLIP}
%     \end{minipage}%
%     \hspace{+0.1mm}%
%     \begin{minipage}[t]{0.3625\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{AuthorKit26/AnonymousSubmission/LaTeX/Figures/M3D.png}
%         \caption*{(c) M3D}
%     \end{minipage}
%     \caption{Similarity matrices between volume and text embeddings across models.}
%     \label{fig:similarity-matrices}
% \end{figure*}


% \begin{figure*}[htbp]
%     \centering
%     \resizebox{0.8\textwidth}{!}{ % Resize the whole group proportionally
%     \begin{minipage}[t]{0.30\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{AuthorKit26/AnonymousSubmission/LaTeX/Figures/3D.png}
%         \caption*{(a) Kaleido-Med}
%     \end{minipage}%
%     \hspace{+0.1mm}%
%     \begin{minipage}[t]{0.3025\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{AuthorKit26/AnonymousSubmission/LaTeX/Figures/Clip.png}
%         \caption*{(b) CT-CLIP}
%     \end{minipage}%
%     \hspace{+0.1mm}%
%     \begin{minipage}[t]{0.3625\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{AuthorKit26/AnonymousSubmission/LaTeX/Figures/M3D.png}
%         \caption*{(c) M3D}
%     \end{minipage}
%     } % end resizebox
%     \caption{\textbf{Cross‑modal similarity matrices for three vision–language models.}  
% Each heat map shows cosine similarity scores in the \([0,1]\) range between volume embeddings (rows) and their paired text‑report embeddings (columns) on the CT‑RATE validation split.  
% \textbf{(a) Kaleido‑Med} displays a sharp block‑diagonal pattern, signalling tight clustering of matched pairs and clear separation from non‑matches.  
% \textbf{(b) CT‑CLIP} exhibits weaker, more diffuse blocks, indicating less precise alignment.  
% \textbf{(c) M3D} appears almost uniform, revealing minimal cross‑modal discrimination.  
% The colour bar (right) maps similarity scores from low (purple) to high (yellow).}
%     \label{fig:similarity-matrices}
% \end{figure*}


\begin{figure}[htbp]
    \centering
    \resizebox{\linewidth}{!}{ % Resize to fit column width
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{AuthorKit26/AnonymousSubmission/LaTeX/Figures/3D.png}
        \caption*{(a) Kaleido-Med}
    \end{minipage}%
    \hspace{0.5mm}%
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{AuthorKit26/AnonymousSubmission/LaTeX/Figures/Clip.png}
        \caption*{(b) CT-CLIP}
    \end{minipage}%
    \hspace{0.5mm}%
    \begin{minipage}[t]{0.38\linewidth}
        \centering
        \includegraphics[width=\linewidth]{AuthorKit26/AnonymousSubmission/LaTeX/Figures/M3D.png}
        \caption*{(c) M3D}
    \end{minipage}
    }
    \caption{Cross‑modal similarity matrices}
    \label{fig:similarity-matrices}
\end{figure}



% Each heat map shows cosine similarity scores \([0,1]\) between volume embeddings (rows) and text-report embeddings (columns) on the CT‑RATE validation split. \textbf{(a)} Kaleido‑Med shows tight clustering; \textbf{(b)} CT‑CLIP has weaker alignment; \textbf{(c)} M3D lacks discrimination.
